Stochastic Bandits for Multi-platform Budget Optimization in Online Advertising

We study the problem of an online advertising system that wants to optimally spend an advertiser's given budget for a campaign across multiple platforms, without knowing the value for showing an ad to the users on those platforms. We model this challenging practical application as a Stochastic Bandits with Knapsacks problem over $T$ rounds of bidding with the set of arms given by the set of distinct bidding $m$-tuples, where $m$ is the number of platforms. We modify the algorithm proposed in Badanidiyuru \emph{et al.,} to extend it to the case of multiple platforms to obtain an algorithm for both the discrete and continuous bid-spaces. Namely, for discrete bid spaces we give an algorithm with regret $O\left(OPT \sqrt {\frac{mn}{B} }+ \sqrt{mn OPT}\right)$, where $OPT$ is the performance of the optimal algorithm that knows the distributions. For continuous bid spaces the regret of our algorithm is $\tilde{O}\left(m^{1/3} \cdot \min\left\{ B^{2/3}, (m T)^{2/3} \right\} \right)$. When restricted to this special-case, this bound improves over Sankararaman and Slivkins in the regime $OPT \ll T$, as is the case in the particular application at hand. Second, we show an $ \Omega\left (\sqrt {m OPT} \right)$ lower bound for the discrete case and an $\Omega\left( m^{1/3} B^{2/3}\right)$ lower bound for the continuous setting, almost matching the upper bounds. Finally, we use a real-world data set from a large internet online advertising company with multiple ad platforms and show that our algorithms outperform common benchmarks and satisfy the required properties warranted in the real-world application.

==> concl.tex <==



==> related_work.tex <==
\subsection{Related Work}\label{sec:relatedwork}

The problem of optimal bidding policies in second price auctions from the perspective of bidders/advertisers can be broadly categorized into four themes.

\paragraph{Budget management with known valuation.} Early approaches to budget management with known valuations (and a single platform) have focused on shading an advertiser's value by a multiplier (often called the ``pacing multiplier''). For example, the work of \cite{rusmevichientong2006, feldman2007budget, hosanagar2008} implement bid shading strategies to maximize the advertisers ROI. What makes this approach appealing, is that the static problem (with known competitor bids) has an optimal solution with a \emph{constant} pacing multipier, so the dynamic approach aims to find this constant. More recent work \cite{cray2007,borgs2007dynamics,balseiro2017budget, conitzer2018pacing, ConitzerKPSSSW2019} have complemented this bid-manipulation literature with equilibrium analysis under the assumption that all advertisers use the same bid-shading approach. 

An alternative to bid modification, is for a platform to restrict the number of auctions that an advertiser participates in. Work by Mehta et al.~\cite{mehta2007adwords} give revenue guarantees for the online matching problem of users showing up over time. Subsequently bidder selection has been applied to multi-objective optimization for Generalized Second Price auctions in e.g. \cite{abrams2008comprehensive,azar2009gsp,goel2010gsp,karande2013pacing}. While the work on bidder selection yields allocations that respect the budget constraint, advertisers are not best-responding to the competition and they can generally improve their allocation by lowering their bids.

\paragraph{Bidding with unknown valuations and no budget constraints.} Feng et al. \cite{feng2018learning} focus on the problem of bidding on a platform without knowing the valuations for users. They model this as a stochastic bandit setting with partial feedback (they only learn the value if the ad won, and the action that the advertiser cares about was taken). They give an online learning algorithm with regret that grows logarithmically in the size of the action space. Their model considers more complex auction environments such as position auctions \cite{V07,EOS07}, though it doesn't take into account multiple platforms or budget constraints.

\paragraph{Budget constrained bidding and unknown valuations.} This line of literature combines the problem settings of the above two themes. More specifically, existing work consider the setting where the valuation as well as the distribution of the competing bids is unknown and focus on optimal bidding strategies that satisfy the specified budget, maximizes the cumulative rewards and learns the valuation of the item. To the best of our knowledge, the problem of learning the optimal bid in second price auctions was first considered by Amin et al. \cite{amin2012budget}. They focus on the discrete bids setting, where the feasible bids belong to a discrete set of bids and formulate the problem as Markov decision process with censored observations. They propose a learning algorithm based on the popular product-limit estimator and demonstrate empirically that their algorithm converges to optimal solution. Tran-Tranh et al. \cite{tran2012knapsack} followed up on the work of \cite{amin2012budget} and provided theoretical guarantees for the algorithm proposed in the later work. More specifically, they assume that the bids are sampled from a discrete distribution in $\{1, \cdots, C\}$ and establish $O(\sqrt{CB})$ regret bounds, where $C$ is the number of feasible bids and $B$ is the total budget. The aforementioned regret bounds depend on some parameters of the competing bids distribution. Flajolet and Jailiet \cite{flajolet2017real} consider a more general variant of the aforementioned problem by relaxing the assumption that the bids come from a discrete set  and proposed an algorithm based on the probabilistic bisection (see \cite{stochastic_root_finder}) and upper confidence bounds (UCB) family of algorithms. They establish $O(\sqrt{T})$ regret bound for the problem under the assumption that budget scales linearly with time, i.e. $B = \Theta(T)$. All three works (\cite{amin2012budget}, \cite{tran2012knapsack} and \cite{flajolet2017real}) in this theme only focus on bidding strategies for a single platform and cannot be easily generalized to the multi-platform setting. 

\paragraph{Stochastic bandits with knapsack constraints. } Stochastic bandits with knapsacks (BwK), introduced in the seminal work of Badanidiyuru et al. \cite{BKS13} is a general framework that considers the standard multi-armed bandit problem under the presence of additional budget/resource constraints in addition to the time horizon constraint. The BwK problem encapsulates a large number of constrained bandit problems that naturally arise in many application domains including dynamic pricing, auction bidding, routing and scheduling. \cite{BKS13, Badanidiyuru:2018} presents two algorithms based respectively on balanced exploration and primal-dual  also used in this work with performances close to the information theoretical optimum. More specifically, they establish a $O(\log(dT)(\sqrt{X \bar{{\sf OPT}}}  + \bar {\sf OPT}\sqrt{m/B}))$, where $X$ is the total number of arms, $d$ is the number of constraints, $B$ is the binding budget constraint and $\bar{\sf{OPT}} $ is a ``reasonable" upper bound on the cumulative optimal reward. A naive generalization of the BwK framework to our problem would result in a combinatorial number of arms ($n^m$ possible bids). Recently, Sankarraman and Slivkins \cite{Karthik-aistats18} extended the BwK framework to combinatorial action sets and established $O(\sqrt{XT})$ regret bounds, which is only optimal only when the cumulative reward is comparable to the length of the time horizon, which is not the case in many online auctions. In this work, we extend the BwK (\cite{BKS13}) framework to propose an optimal bidding strategy with performances guarantees that are near optimal even when the cumulative reward is much smaller in comparison to length of the time horizon. 

The BwK framework \cite{BKS13} also has  been extended with near-optimal regret bounds to  contextual bandits (see \cite{pmlr-v35-badanidiyuru14,CBwK-colt16,CBwK-nips16}), settings with concave reward functions and convex constraints (see \cite{AD14}). Adversarial bandits with knapsack are also  extended in \cite{Immorlica19} to the combinatorial semi-bandit, contextual, and convex optimization settings.  However, these problem settings are not immediately applicable to our problem.
